Two Souls in an Adversarial Image: Towards Universal Adversarial Example Detection using Multi-view Inconsistency

In the evasion attacks against deep neural networks (DNN), the attacker generates adversarial instances that are visually indistinguishable from benign samples and sends them to the target DNN to trigger misclassifications. In this paper, we propose a novel multi-view adversarial image detector, namely Argos, based on a novel observation. That is, there exist two "souls" in an adversarial instance, i.e., the visually unchanged content, which corresponds to the true label, and the added invisible perturbation, which corresponds to the misclassified label. Such inconsistencies could be further amplified through an autoregressive generative approach that generates images with seed pixels selected from the original image, a selected label, and pixel distributions learned from the training data. The generated images (i.e., the "views") will deviate significantly from the original one if the label is adversarial, demonstrating inconsistencies that Argos expects to detect. To this end, Argos first amplifies the discrepancies between the visual content of an image and its misclassified label induced by the attack using a set of regeneration mechanisms and then identifies an image as adversarial if the reproduced views deviate to a preset degree. Our experimental results show that Argos significantly outperforms two representative adversarial detectors in both detection accuracy and robustness against six well-known adversarial attacks. Code is available at: https://github.com/sohaib730/Argos-Adversarial_Detection

==> draft.tex <==

For our detection scheme, one key objective is to estimate distribution of input images $p(x)$. Eventually, we will be looking to partially generate images in ordered fashion, so auto regressive generative model are in particular more suitable.  The Autoregressive Image generative techniques  fully factorizes the probability density function on an image x over all its sub-pixels (color channels in a pixel) as:
\begin{equation}
p(x) = \prod_{i=1}^{n^2}p(x_{i}|x_{1},....x_{i-1}) = \prod_{i=1}^{n^2}p(x_{i}|x_{<i})
\end{equation}
The pixel dependencies are in raster scan order (row by row and pixel by pixel within
every row). Every pixel therefore depends on all the pixels above and to the left of it, and not on any
of other pixels. Such that $x_{<i}=[x_{1},x_{2},..,x_{i-1}]$ denotes the vector of random variables with index less than i.

The difference between different auto regressive generative techniques  NADE [14], RIDE [26] and PixelCNN[] is the way the conditional distributions $p(xi|x_{<i})$ are constructed. 
The PixelCNN, introduced by van den Oord et al. (2016b), is a best known generative model of images with a tractable likelihood. In PixelCNN every conditional distribution is modelled by a convolutional neural network and it's weights are shared among all pixels.


PixelCNN can easily be extended to approximate image distribution conditioned on label information [conditional PixelCNN]. Given an image label represented as a vector $c$, it seeks to model the conditional
distribution $p(x|c)$ of images suiting this description. Formally the conditional PixelCNN models the following distribution:
\begin{equation}
p(x|y) = \prod_{i=1}^{n^2}p(x_{i}|x_{1},....x_{i-1},y)   
\end{equation}
One could expect that conditioning the image generation on class label could significantly improve
the log-likelihood results, however in [conditional pixelCNN] they did not observe big differences. On the other hand, as noted
in [27][condtitional PixelCNN], they observed great improvements in the visual quality of the generated samples. 

Due to limited space, we are not giving details about PixelCNN model architecture or learning procedure. To get more insight, we will encourage readers to look at previous work. [pixelRNN][Conditional PixelCNN] and [PixelCNN++]. Till date, the best variant of PixelCNN is pixelCNN++[] that  contains a number of modifications to the original model that both simplify its structure and improve its performance. Hence, we will be using PixelCNN++ to model class conditional image distribution $p(x|y)$


\subsection{View Generation Scheme}






We will be using autoregressive generative process, to generate all views, whose input is classified label $\hat{y}$ and i number of seed pixels and $\{x_1,x_2...x_i\}$. The only difference among different generated views $(G_1,..G_5)$, is in $G_1$ classified label information will be more dominant to enhance dissimilarity as shown Figure, Whereas, in $G_4$ likelihood distribution of seed pixels will be more dominant. Then in $G_2,G_3$ both factors will play a role in enhancing dissimilarity. 

Based on the above mentioned desirable properties our view generation scheme is as follows. The autoregressive(AR) generator is first trained on clean training images to learn class conditional likelihood distribution $P(x|Label)$. To generate multiple views of input candidate image that we want to detect, the AR generator takes classified label and some rows of candidate image(we call them as seed pixels) as input. The only difference among first four generated views is the number of seed pixels provided to AR generator. As shown in figure (a), for an input image with its classified label. The grey rows in $(G_1,..G_5)$ represents the number of pixels that will be generated in each view. For input image of dimension n by n with n=32. The first view $G_1$ is generated by taking first 8 rows of input candidate image as seed pixels. For $G_2$ first 12 rows of input image will be seed pixels. Both in $G_1,G_2$ the number of seed pixels are less. Thus the generated pixels will contain classified label object as shown in Figure. For Similarly, to get $G_3,G_4$, first 16 and 24 rows respectively of input image will act as seed. Here number of seed pixels are high and as a result the generated pixels are determined by seed pixels likelihood distribution as shown in Figure. At the end last view $G_5$ only contain different rows of input and previously generated views $(G_1,..G_4)$. First 8 rows are taken from input image. Then row 9-12, 13-16, 17-24 and 25-32 are taken from $G_1, G_2, G_3$ and $G_4$ respectively. 

\subsection{Detectors}
We have created five different views for input candidate image that we want to detect. There are number of ways we can obtain consistency among different views. Therefore, we use different detection schemes depending upon complexity of the datasets. As, the complexity of datasets affects the quality of generated views. 

We get best quality of generated views when input images only contain classification object with no background. Moreover, each object appearance is similar in all images. Both assumptions are quite practical when we look at traffic sign board dataset in figure. Also it can be viewed the all generated views are nearly identical. Therefore, seperating clean from adversarial is simpler just by taking euclidean distance between candidate sample x and generated view $G_5$. Although, we can use other view like $G_1$ but generation $G_5$ is computationaly efficient. Since $G_5$ consist of few rows from each view $G1..G4$ which can be computed in parallel. The detection criteria is as follows:

\begin{equation}
    \left \| x-G_5(x,F(x) \right \|_2 \overset{adv.}{\underset{Clean}{\gtrless}} \theta
\end{equation}

For slightly complex datasets, we again assume object bounding boxes/location is known. So we can pass the cropped image that only contain object with little background for view generation. However, here each object can have varied appaearance in different samples. The generated will mostly contain the classified label object but it's shape an orientation will not match with the appearance in candidate image. Therefore, for such type of datasets we look into representation vector $h(.)$ and classifier output F(.) to estimate consistence among different views. Since all generated views contain major features of oclassified, we expect representation vector of candidate image h(x) and generated view $h(G_5(x,\hat{y}))$ will be close. On the other hand, for adversarial image the added perturbation is already enhanced in $G_3,G_4$ and then it will further amplified when we look into representation vector, so h(x') and $h(G_5(x',\hat{y}))$ will be far apart. The other parameter that can be more helpful to detect adversarial samples with very small perturbation is the dissimilarity among classified label from all views i.e $F(x), F(G_1) ...F_(G_5)$. Adversarial examples that lie near the decision boundry, the generated views that are around that candidate image might have different classification. Although, there could be some clean samples who are at the decision boundry, but we found drop in clean detection is less as compare to gain in adversarial detection. To estimate similarity among classification label of all generated views and candidate sample, we use Entropy score. Then input sample is adversarial if one of the following condition is true otherwise clean:

\begin{equation}
\begin{split}
\label{detector2}
\left \|  h(x) - h(G_5(x,F(x)))\right \|_2 \overset{adv.}  > \theta_1\\
Or,\\
Entropy[F(x),F(G_1(x,F(x)))..F(G_5(x,F(x)))] \overset{adv.}  > \theta_2
\end{split}
\end{equation}
Although, above mentioned assumption of known object location is practical. But for completness we also look at the dataset where objects are not bounded as shown in Row 3 of Figure. In this case quality of generated views will not visually match with candidate image. However, the generated views will still contain the required features. For detection  


==> preliminary.tex <==
\section{Preliminaries}
\label{sec:pre}

\subsection{Notations}
We represent clean samples as $(x,y)$, where $x$ is n by n dimensional input image and $y$ is the true Label. The subpixels of an image $x$ are represented as $x_i$. We represent classification network as $F(.)$, such that $F(x)$ represents the output label for input image $x$. The loss function of a classifier network $F(.)$ is represented as $L(\theta,x,y)$, where $\theta$ are the network's weights. We represent penultimate layer output of the network $F(.)$, also know as representation vector, as $h(x)$.

For any clean sample $(x,y)$, whose classified output is $F(x)=y$, the corresponding adversarial example $x'$ gives $F(x') \neq y$ and is within certain $L_p$ distance from x i.e. $\left \| x-x' \right \|_p \leq \epsilon $,  as given by Goodfellow et al. \cite{goodfellow2014explaining}. Also, we will specify $\epsilon$ in terms of pixel values in the range [0, 255]. 

\subsection{Auto Regressive Image Generative Model}
For our detection scheme, one key objective is to estimate distribution of input images $p(x)$. Eventually, we will be looking to partially generate images in ordered fashion, so auto regressive generative model are in particular more suitable.  The Autoregressive Image generative techniques fully factorizes the probability density function on an image $x$ over all its sub-pixels (color channels in a pixel) as:
\begin{equation}
p(x) = \prod_{i=1}^{n^2}p(x_{i}|x_{1},....x_{i-1}) = \prod_{i=1}^{n^2}p(x_{i}|x_{<i})
\end{equation}
The pixel dependencies are in raster scan order (row by row and pixel by pixel within
every row). Every pixel therefore depends on all the pixels above and to the left of it, and not on any
of other pixels. Such that $x_{<i}=[x_{1},x_{2},..,x_{i-1}]$ denotes the vector of random variables with index less than $i$.

The difference between different auto regressive generative techniques NADE [14], RIDE [26] and PixelCNN[] is the way the conditional distributions $p(xi|x_{<i})$ are constructed. 
The PixelCNN, introduced by van den Oord et al. (2016b), is a best known generative model of images with a tractable likelihood. In PixelCNN every conditional distribution is modelled by a convolutional neural network and it's weights are shared among all pixels.


PixelCNN can easily be extended to approximate image distribution conditioned on label information [conditional PixelCNN]. Given an image label represented as a vector $c$, it seeks to model the conditional
distribution $p(x|c)$ of images suiting this description. Formally the conditional PixelCNN models the following distribution:
\begin{equation}
p(x|y) = \prod_{i=1}^{n^2}p(x_{i}|x_{1},....x_{i-1},y)   
\end{equation}
One could expect that conditioning the image generation on class label could significantly improve
the log-likelihood results, however in [conditional pixelCNN] they did not observe big differences. On the other hand, as noted
in [27][condtitional PixelCNN], they observed great improvements in the visual quality of the generated samples. 

Due to limited space, we are not giving details about PixelCNN model architecture or learning procedure. To get more insight, we will encourage readers to look at previous work. [pixelRNN][Conditional PixelCNN] and [PixelCNN++]. Till date, the best variant of PixelCNN is pixelCNN++[] that  contains a number of modifications to the original model that both simplify its structure and improve its performance. Hence, we will be using PixelCNN++ to model class conditional image distribution $p(x|y)$




